Heterogeneous Hypergraph Embedding for Graph Classification

Recently, graph neural networks have been widely used for network embedding because of their prominent performance in pairwise relationship learning. In the real world, a more natural and common situation is the coexistence of pairwise relationships and complex non-pairwise relationships, which is, however, rarely studied. In light of this, we propose a graph neural network-based representation learning framework for heterogeneous hypergraphs, an extension of conventional graphs, which can well characterize multiple non-pairwise relations. Our framework first projects the heterogeneous hypergraph into a series of snapshots and then we take the Wavelet basis to perform localized hypergraph convolution. Since the Wavelet basis is usually much sparser than the Fourier basis, we develop an efficient polynomial approximation to the basis to replace the time-consuming Laplacian decomposition. Extensive evaluations have been conducted and the experimental results show the superiority of our method. In addition to the standard tasks of network embedding evaluation such as node classification, we also apply our method to the task of spammers detection and the superior performance of our framework shows that relationships beyond pairwise are also advantageous in the spammer detection.

==> main <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{43}

%%% ====================================================================
%%% NOTE TO THE USER: you can override these defaults by providing
%%% customized versions of any of these macros before the \bibliography
%%% command.  Each of them MUST provide its own final punctuation,
%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
%%% do not use final punctuation, in order to avoid confusing it with
%%% the Web address.
%%%
%%% To suppress output of a particular field, define its macro to expand
%%% to an empty string, or better, \unskip, like this:
%%%
%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
%%%
%%% \def \showDOI #1{\unskip}           % plain TeX syntax
%%%
%%% ====================================================================

\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
\ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
\ifx \showURL      \undefined \def \showURL       {\relax}        \fi
% The following commands are used for tagged output and should be
% invisible to TeX
\providecommand\bibfield[2]{#2}
\providecommand\bibinfo[2]{#2}
\providecommand\natexlab[1]{#1}
\providecommand\showeprint[2][]{arXiv:#2}

\bibitem[\protect\citeauthoryear{Blondel, Guillaume, Lambiotte, and
  Lefebvre}{Blondel et~al\mbox{.}}{2008}]%
        {blondel2008fast}
\bibfield{author}{\bibinfo{person}{Vincent~D Blondel},
  \bibinfo{person}{Jean-Loup Guillaume}, \bibinfo{person}{Renaud Lambiotte},
  {and} \bibinfo{person}{Etienne Lefebvre}.} \bibinfo{year}{2008}\natexlab{}.
\newblock \showarticletitle{Fast unfolding of communities in large networks}.
\newblock \bibinfo{journal}{\emph{Journal of statistical mechanics: theory and
  experiment}} \bibinfo{volume}{2008}, \bibinfo{number}{10}
  (\bibinfo{year}{2008}), \bibinfo{pages}{P10008}.
\newblock


\bibitem[\protect\citeauthoryear{Bretto}{Bretto}{2013}]%
        {Bretto2013}
\bibfield{author}{\bibinfo{person}{Alain Bretto}.}
  \bibinfo{year}{2013}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{Applications of Hypergraph Theory: A Brief
  Overview}}.
\newblock \bibinfo{publisher}{Springer International Publishing},
  \bibinfo{address}{Heidelberg}, \bibinfo{pages}{111--116}.
\newblock
\showISBNx{978-3-319-00080-0}
\urldef\tempurl%
\url{https://doi.org/10.1007/978-3-319-00080-0_7}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Bruna, Zaremba, Szlam, and LeCun}{Bruna
  et~al\mbox{.}}{2014}]%
        {bruna2013spectral}
\bibfield{author}{\bibinfo{person}{Joan Bruna}, \bibinfo{person}{Wojciech
  Zaremba}, \bibinfo{person}{Arthur Szlam}, {and} \bibinfo{person}{Yann
  LeCun}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Spectral networks and locally connected networks on
  graphs}.
\newblock \bibinfo{journal}{\emph{ICLR}} (\bibinfo{year}{2014}).
\newblock


\bibitem[\protect\citeauthoryear{Chen, Yin, Chen, Wang, Li, and Hu}{Chen
  et~al\mbox{.}}{2020a}]%
        {chen2020social}
\bibfield{author}{\bibinfo{person}{Hongxu Chen}, \bibinfo{person}{Hongzhi Yin},
  \bibinfo{person}{Tong Chen}, \bibinfo{person}{Weiqing Wang},
  \bibinfo{person}{Xue Li}, {and} \bibinfo{person}{Xia Hu}.}
  \bibinfo{year}{2020}\natexlab{a}.
\newblock \showarticletitle{Social Boosted Recommendation with Folded Bipartite
  Network Embedding}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Knowledge and Data
  Engineering}} (\bibinfo{year}{2020}).
\newblock


\bibitem[\protect\citeauthoryear{Chen, Yin, Sun, Chen, Gabrys, and Musial}{Chen
  et~al\mbox{.}}{2020b}]%
        {chen2020hypergraph}
\bibfield{author}{\bibinfo{person}{Hongxu Chen}, \bibinfo{person}{Hongzhi Yin},
  \bibinfo{person}{Xiangguo Sun}, \bibinfo{person}{Tong Chen},
  \bibinfo{person}{Bogdan Gabrys}, {and} \bibinfo{person}{Katarzyna Musial}.}
  \bibinfo{year}{2020}\natexlab{b}.
\newblock \showarticletitle{Multi-level Graph Convolutional Networks for
  Cross-platform Anchor Link Prediction}. In \bibinfo{booktitle}{\emph{KDD20}}.
\newblock


\bibitem[\protect\citeauthoryear{Chen, Yin, Wang, Wang, Nguyen, and Li}{Chen
  et~al\mbox{.}}{2018}]%
        {chen2018pme}
\bibfield{author}{\bibinfo{person}{Hongxu Chen}, \bibinfo{person}{Hongzhi Yin},
  \bibinfo{person}{Weiqing Wang}, \bibinfo{person}{Hao Wang},
  \bibinfo{person}{Quoc Viet~Hung Nguyen}, {and} \bibinfo{person}{Xue Li}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{PME}: projected metric embedding on heterogeneous
  networks for link prediction}. In \bibinfo{booktitle}{\emph{Proceedings of
  the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data
  Mining}}. ACM, \bibinfo{pages}{1177--1186}.
\newblock


\bibitem[\protect\citeauthoryear{Chu, Feng, and Guo}{Chu et~al\mbox{.}}{2018}]%
        {chu2018social}
\bibfield{author}{\bibinfo{person}{Yunfei Chu}, \bibinfo{person}{Chunyan Feng},
  {and} \bibinfo{person}{Caili Guo}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Social-Guided Representation Learning for Images
  via Deep Heterogeneous Hypergraph Embedding}. IEEE,
  \bibinfo{publisher}{ICME}.
\newblock


\bibitem[\protect\citeauthoryear{Defferrard, Bresson, and
  Vandergheynst}{Defferrard et~al\mbox{.}}{2016}]%
        {defferrard2016convolutional}
\bibfield{author}{\bibinfo{person}{Micha{\"e}l Defferrard},
  \bibinfo{person}{Xavier Bresson}, {and} \bibinfo{person}{Pierre
  Vandergheynst}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Convolutional neural networks on graphs with fast
  localized spectral filtering}. In \bibinfo{booktitle}{\emph{NeurIPS}}.
  \bibinfo{pages}{3844--3852}.
\newblock


\bibitem[\protect\citeauthoryear{Dong, Chawla, and Swami}{Dong
  et~al\mbox{.}}{[n.d.]}]%
        {metapath2vec}
\bibfield{author}{\bibinfo{person}{Yuxiao Dong}, \bibinfo{person}{Nitesh~V
  Chawla}, {and} \bibinfo{person}{Ananthram Swami}.}
  \bibinfo{year}{[n.d.]}\natexlab{}.
\newblock \showarticletitle{metapath2vec: Scalable representation learning for
  heterogeneous networks}. In \bibinfo{booktitle}{\emph{SIGKDD17}}.
\newblock


\bibitem[\protect\citeauthoryear{Donnat, Zitnik, Hallac, and Leskovec}{Donnat
  et~al\mbox{.}}{2018}]%
        {donnat2018learning}
\bibfield{author}{\bibinfo{person}{Claire Donnat}, \bibinfo{person}{Marinka
  Zitnik}, \bibinfo{person}{David Hallac}, {and} \bibinfo{person}{Jure
  Leskovec}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Learning structural node embeddings via diffusion
  wavelets}. In \bibinfo{booktitle}{\emph{Proceedings of the 24th ACM SIGKDD
  International Conference on Knowledge Discovery \& Data Mining}}. ACM,
  \bibinfo{pages}{1320--1329}.
\newblock


\bibitem[\protect\citeauthoryear{Feng, You, Zhang, Ji, and Gao}{Feng
  et~al\mbox{.}}{2019}]%
        {feng2019hypergraph}
\bibfield{author}{\bibinfo{person}{Yifan Feng}, \bibinfo{person}{Haoxuan You},
  \bibinfo{person}{Zizhao Zhang}, \bibinfo{person}{Rongrong Ji}, {and}
  \bibinfo{person}{Yue Gao}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Hypergraph neural networks}. In
  \bibinfo{booktitle}{\emph{AAAI}}. \bibinfo{pages}{3558--3565}.
\newblock


\bibitem[\protect\citeauthoryear{Gao, Wang, Zha, Shen, Li, and Wu}{Gao
  et~al\mbox{.}}{2012}]%
        {gao2012visual}
\bibfield{author}{\bibinfo{person}{Yue Gao}, \bibinfo{person}{Meng Wang},
  \bibinfo{person}{Zheng-Jun Zha}, \bibinfo{person}{Jialie Shen},
  \bibinfo{person}{Xuelong Li}, {and} \bibinfo{person}{Xindong Wu}.}
  \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{Visual-textual joint relevance learning for
  tag-based social image search}.
\newblock \bibinfo{journal}{\emph{TIP}} \bibinfo{volume}{22},
  \bibinfo{number}{1} (\bibinfo{year}{2012}), \bibinfo{pages}{363--376}.
\newblock


\bibitem[\protect\citeauthoryear{Grover and Leskovec}{Grover and
  Leskovec}{2016}]%
        {node2vec}
\bibfield{author}{\bibinfo{person}{Aditya Grover} {and} \bibinfo{person}{Jure
  Leskovec}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{node2vec: Scalable feature learning for networks}.
  In \bibinfo{booktitle}{\emph{KDD}}. ACM.
\newblock


\bibitem[\protect\citeauthoryear{Hamilton, Ying, and Leskovec}{Hamilton
  et~al\mbox{.}}{2017}]%
        {hamilton2017inductive}
\bibfield{author}{\bibinfo{person}{Will Hamilton}, \bibinfo{person}{Zhitao
  Ying}, {and} \bibinfo{person}{Jure Leskovec}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Inductive representation learning on large graphs}.
  In \bibinfo{booktitle}{\emph{NeurIPS}}. \bibinfo{pages}{1024--1034}.
\newblock


\bibitem[\protect\citeauthoryear{Huang, Liu, and Metaxas}{Huang
  et~al\mbox{.}}{2009}]%
        {huang2009video}
\bibfield{author}{\bibinfo{person}{Yuchi Huang}, \bibinfo{person}{Qingshan
  Liu}, {and} \bibinfo{person}{Dimitris Metaxas}.}
  \bibinfo{year}{2009}\natexlab{}.
\newblock \showarticletitle{Video object segmentation by hypergraph cut}. In
  \bibinfo{booktitle}{\emph{CVPR}}. \bibinfo{pages}{1738--1745}.
\newblock


\bibitem[\protect\citeauthoryear{Hwang, Tian, Kuangy, and Kocher}{Hwang
  et~al\mbox{.}}{2008}]%
        {hwang2008learning}
\bibfield{author}{\bibinfo{person}{TaeHyun Hwang}, \bibinfo{person}{Ze Tian},
  \bibinfo{person}{Rui Kuangy}, {and} \bibinfo{person}{Jean-Pierre Kocher}.}
  \bibinfo{year}{2008}\natexlab{}.
\newblock \showarticletitle{Learning on weighted hypergraphs to integrate
  protein interactions and gene expressions for cancer outcome prediction}. In
  \bibinfo{booktitle}{\emph{ICDM}}. \bibinfo{pages}{293--302}.
\newblock


\bibitem[\protect\citeauthoryear{Jiang, Wei, Feng, Cao, and Gao}{Jiang
  et~al\mbox{.}}{2019}]%
        {jiang2019dynamic}
\bibfield{author}{\bibinfo{person}{Jianwen Jiang}, \bibinfo{person}{Yuxuan
  Wei}, \bibinfo{person}{Yifan Feng}, \bibinfo{person}{Jingxuan Cao}, {and}
  \bibinfo{person}{Yue Gao}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Dynamic hypergraph neural networks}.
  \bibinfo{publisher}{IJCAI}.
\newblock


\bibitem[\protect\citeauthoryear{Kipf and Welling}{Kipf and Welling}{2016}]%
        {kipf2016semi}
\bibfield{author}{\bibinfo{person}{Thomas~N Kipf} {and} \bibinfo{person}{Max
  Welling}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Semi-supervised classification with graph
  convolutional networks}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1609.02907}}
  (\bibinfo{year}{2016}).
\newblock


\bibitem[\protect\citeauthoryear{Liu, Sun, Ni, Cao, Luo, Liu, and Fu}{Liu
  et~al\mbox{.}}{2020}]%
        {sunspammer2020}
\bibfield{author}{\bibinfo{person}{Bo Liu}, \bibinfo{person}{Xiangguo Sun},
  \bibinfo{person}{Zeyang Ni}, \bibinfo{person}{Jiuxin Cao},
  \bibinfo{person}{Junzhou Luo}, \bibinfo{person}{Benyuan Liu}, {and}
  \bibinfo{person}{Xinwen Fu}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Co-Detection of Crowdturﬁng Microblogs and
  Spammers in Online Social Networks}.
\newblock \bibinfo{journal}{\emph{World Wide Web Journal}}
  (\bibinfo{year}{2020}).
\newblock


\bibitem[\protect\citeauthoryear{Liu, Liu, Zhang, and Ma}{Liu
  et~al\mbox{.}}{2016}]%
        {liu2016pay}
\bibfield{author}{\bibinfo{person}{Yuli Liu}, \bibinfo{person}{Yiqun Liu},
  \bibinfo{person}{Min Zhang}, {and} \bibinfo{person}{Shaoping Ma}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Pay Me and I'll Follow You: Detection of
  Crowdturfing Following Activities in Microblog Environment.}. In
  \bibinfo{booktitle}{\emph{IJCAI}}. \bibinfo{pages}{3789--3796}.
\newblock


\bibitem[\protect\citeauthoryear{McCallum, Nigam, Rennie, and Seymore}{McCallum
  et~al\mbox{.}}{2000}]%
        {mccallum2000automating}
\bibfield{author}{\bibinfo{person}{Andrew~Kachites McCallum},
  \bibinfo{person}{Kamal Nigam}, \bibinfo{person}{Jason Rennie}, {and}
  \bibinfo{person}{Kristie Seymore}.} \bibinfo{year}{2000}\natexlab{}.
\newblock \showarticletitle{Automating the construction of internet portals
  with machine learning}.
\newblock \bibinfo{journal}{\emph{Information Retrieval}} \bibinfo{volume}{3},
  \bibinfo{number}{2} (\bibinfo{year}{2000}), \bibinfo{pages}{127--163}.
\newblock


\bibitem[\protect\citeauthoryear{Mikolov, Sutskever, Chen, Corrado, and
  Dean}{Mikolov et~al\mbox{.}}{2013}]%
        {mikolov2013distributed}
\bibfield{author}{\bibinfo{person}{Tomas Mikolov}, \bibinfo{person}{Ilya
  Sutskever}, \bibinfo{person}{Kai Chen}, \bibinfo{person}{Greg~S Corrado},
  {and} \bibinfo{person}{Jeff Dean}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{Distributed representations of words and phrases
  and their compositionality}. In \bibinfo{booktitle}{\emph{NIPS}}.
\newblock


\bibitem[\protect\citeauthoryear{Monti, Boscaini, Masci, Rodola, Svoboda, and
  Bronstein}{Monti et~al\mbox{.}}{2017}]%
        {monti2017geometric}
\bibfield{author}{\bibinfo{person}{Federico Monti}, \bibinfo{person}{Davide
  Boscaini}, \bibinfo{person}{Jonathan Masci}, \bibinfo{person}{Emanuele
  Rodola}, \bibinfo{person}{Jan Svoboda}, {and} \bibinfo{person}{Michael~M
  Bronstein}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Geometric deep learning on graphs and manifolds
  using mixture model cnns}. In \bibinfo{booktitle}{\emph{CVPR}}.
  \bibinfo{pages}{5115--5124}.
\newblock


\bibitem[\protect\citeauthoryear{Neelima and Raghavendra}{Neelima and
  Raghavendra}{2012}]%
        {neelima2012effective}
\bibfield{author}{\bibinfo{person}{B Neelima} {and} \bibinfo{person}{Prakash~S
  Raghavendra}.} \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{Effective sparse matrix representation for the GPU
  architectures}.
\newblock \bibinfo{journal}{\emph{International Journal of Computer Science,
  Engineering and Applications}} \bibinfo{volume}{2}, \bibinfo{number}{2}
  (\bibinfo{year}{2012}), \bibinfo{pages}{151}.
\newblock


\bibitem[\protect\citeauthoryear{Niepert, Ahmed, and Kutzkov}{Niepert
  et~al\mbox{.}}{2016}]%
        {niepert2016learning}
\bibfield{author}{\bibinfo{person}{Mathias Niepert}, \bibinfo{person}{Mohamed
  Ahmed}, {and} \bibinfo{person}{Konstantin Kutzkov}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Learning convolutional neural networks for graphs}.
  In \bibinfo{booktitle}{\emph{ICML}}. \bibinfo{pages}{2014--2023}.
\newblock


\bibitem[\protect\citeauthoryear{Perozzi, Al-Rfou, and Skiena}{Perozzi
  et~al\mbox{.}}{2014}]%
        {perozzi2014deepwalk}
\bibfield{author}{\bibinfo{person}{Bryan Perozzi}, \bibinfo{person}{Rami
  Al-Rfou}, {and} \bibinfo{person}{Steven Skiena}.}
  \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Deepwalk: Online learning of social
  representations}. In \bibinfo{booktitle}{\emph{KDD}}. ACM,
  \bibinfo{pages}{701--710}.
\newblock


\bibitem[\protect\citeauthoryear{Sen, Namata, Bilgic, Getoor, Galligher, and
  Eliassi-Rad}{Sen et~al\mbox{.}}{2008}]%
        {sen2008collective}
\bibfield{author}{\bibinfo{person}{Prithviraj Sen}, \bibinfo{person}{Galileo
  Namata}, \bibinfo{person}{Mustafa Bilgic}, \bibinfo{person}{Lise Getoor},
  \bibinfo{person}{Brian Galligher}, {and} \bibinfo{person}{Tina Eliassi-Rad}.}
  \bibinfo{year}{2008}\natexlab{}.
\newblock \showarticletitle{Collective classification in network data}.
\newblock \bibinfo{journal}{\emph{AI magazine}} \bibinfo{volume}{29},
  \bibinfo{number}{3} (\bibinfo{year}{2008}), \bibinfo{pages}{93--93}.
\newblock


\bibitem[\protect\citeauthoryear{Sun, Han, Yan, Yu, and Wu}{Sun
  et~al\mbox{.}}{2011}]%
        {sun2011pathsim}
\bibfield{author}{\bibinfo{person}{Yizhou Sun}, \bibinfo{person}{Jiawei Han},
  \bibinfo{person}{Xifeng Yan}, \bibinfo{person}{Philip~S Yu}, {and}
  \bibinfo{person}{Tianyi Wu}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{Pathsim: Meta path-based top-k similarity search in
  heterogeneous information networks}.
\newblock \bibinfo{journal}{\emph{VLDB}} \bibinfo{volume}{4},
  \bibinfo{number}{11} (\bibinfo{year}{2011}), \bibinfo{pages}{992--1003}.
\newblock


\bibitem[\protect\citeauthoryear{Tang, Qu, and Mei}{Tang
  et~al\mbox{.}}{2015a}]%
        {tang2015pte}
\bibfield{author}{\bibinfo{person}{Jian Tang}, \bibinfo{person}{Meng Qu}, {and}
  \bibinfo{person}{Qiaozhu Mei}.} \bibinfo{year}{2015}\natexlab{a}.
\newblock \showarticletitle{{PTE}: Predictive text embedding through
  large-scale heterogeneous text networks}. In \bibinfo{booktitle}{\emph{KDD}}.
\newblock


\bibitem[\protect\citeauthoryear{Tang, Qu, Wang, Zhang, Yan, and Mei}{Tang
  et~al\mbox{.}}{2015b}]%
        {line}
\bibfield{author}{\bibinfo{person}{Jian Tang}, \bibinfo{person}{Meng Qu},
  \bibinfo{person}{Mingzhe Wang}, \bibinfo{person}{Ming Zhang},
  \bibinfo{person}{Jun Yan}, {and} \bibinfo{person}{Qiaozhu Mei}.}
  \bibinfo{year}{2015}\natexlab{b}.
\newblock \showarticletitle{Line: Large-scale information network embedding}.
  In \bibinfo{booktitle}{\emph{WWW}}.
\newblock


\bibitem[\protect\citeauthoryear{Tu, Cui, Wang, Wang, and Zhu}{Tu
  et~al\mbox{.}}{2018}]%
        {tu2018structural}
\bibfield{author}{\bibinfo{person}{Ke Tu}, \bibinfo{person}{Peng Cui},
  \bibinfo{person}{Xiao Wang}, \bibinfo{person}{Fei Wang}, {and}
  \bibinfo{person}{Wenwu Zhu}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Structural deep embedding for hyper-networks}.
  \bibinfo{publisher}{AAAI}.
\newblock


\bibitem[\protect\citeauthoryear{Veli{\v{c}}kovi{\'c}, Cucurull, Casanova,
  Romero, Lio, and Bengio}{Veli{\v{c}}kovi{\'c} et~al\mbox{.}}{2018}]%
        {velivckovic2017graph}
\bibfield{author}{\bibinfo{person}{Petar Veli{\v{c}}kovi{\'c}},
  \bibinfo{person}{Guillem Cucurull}, \bibinfo{person}{Arantxa Casanova},
  \bibinfo{person}{Adriana Romero}, \bibinfo{person}{Pietro Lio}, {and}
  \bibinfo{person}{Yoshua Bengio}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Graph attention networks}.
\newblock \bibinfo{journal}{\emph{ICLR}} (\bibinfo{year}{2018}).
\newblock


\bibitem[\protect\citeauthoryear{Wang, Zhang, and Shi}{Wang
  et~al\mbox{.}}{2019}]%
        {wang2019hyperbolic}
\bibfield{author}{\bibinfo{person}{Xiao Wang}, \bibinfo{person}{Yiding Zhang},
  {and} \bibinfo{person}{Chuan Shi}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Hyperbolic Heterogeneous Information Network
  Embedding}. AAAI.
\newblock


\bibitem[\protect\citeauthoryear{Wu, Shu, Huang, and Yuan}{Wu
  et~al\mbox{.}}{2015}]%
        {wu2015social}
\bibfield{author}{\bibinfo{person}{Fangzhao Wu}, \bibinfo{person}{Jinyun Shu},
  \bibinfo{person}{Yongfeng Huang}, {and} \bibinfo{person}{Zhigang Yuan}.}
  \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Social spammer and spam message co-detection in
  microblogging with social context regularization}. In
  \bibinfo{booktitle}{\emph{CIKM}}. \bibinfo{pages}{1601--1610}.
\newblock


\bibitem[\protect\citeauthoryear{Xu, Shen, Cao, Qiu, and Cheng}{Xu
  et~al\mbox{.}}{2019}]%
        {xu2019graph}
\bibfield{author}{\bibinfo{person}{Bingbing Xu}, \bibinfo{person}{Huawei Shen},
  \bibinfo{person}{Qi Cao}, \bibinfo{person}{Yunqi Qiu}, {and}
  \bibinfo{person}{Xueqi Cheng}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Graph Wavelet Neural Network}.
\newblock \bibinfo{journal}{\emph{ICLR}} (\bibinfo{year}{2019}).
\newblock


\bibitem[\protect\citeauthoryear{Yadati, Nimishakavi, Yadav, Nitin, Louis, and
  Talukdar}{Yadati et~al\mbox{.}}{2019}]%
        {yadati2019hypergcn}
\bibfield{author}{\bibinfo{person}{Naganand Yadati}, \bibinfo{person}{Madhav
  Nimishakavi}, \bibinfo{person}{Prateek Yadav}, \bibinfo{person}{Vikram
  Nitin}, \bibinfo{person}{Anand Louis}, {and} \bibinfo{person}{Partha
  Talukdar}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{HyperGCN: A New Method For Training Graph
  Convolutional Networks on Hypergraphs}. \bibinfo{publisher}{NeurIPS}.
\newblock


\bibitem[\protect\citeauthoryear{Yin, Wang, Zheng, Li, Yang, and Zhou}{Yin
  et~al\mbox{.}}{2019}]%
        {yin2019social}
\bibfield{author}{\bibinfo{person}{Hongzhi Yin}, \bibinfo{person}{Qinyong
  Wang}, \bibinfo{person}{Kai Zheng}, \bibinfo{person}{Zhixu Li},
  \bibinfo{person}{Jiali Yang}, {and} \bibinfo{person}{Xiaofang Zhou}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Social influence-based group representation
  learning for group recommendation}. In \bibinfo{booktitle}{\emph{ICDE}}.
  IEEE, \bibinfo{pages}{566--577}.
\newblock


\bibitem[\protect\citeauthoryear{Yin, Wang, Wang, Chen, and Zhou}{Yin
  et~al\mbox{.}}{2017}]%
        {yin2017spatial}
\bibfield{author}{\bibinfo{person}{Hongzhi Yin}, \bibinfo{person}{Weiqing
  Wang}, \bibinfo{person}{Hao Wang}, \bibinfo{person}{Ling Chen}, {and}
  \bibinfo{person}{Xiaofang Zhou}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Spatial-aware hierarchical collaborative deep
  learning for POI recommendation}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Knowledge and Data
  Engineering}} \bibinfo{volume}{29}, \bibinfo{number}{11}
  (\bibinfo{year}{2017}), \bibinfo{pages}{2537--2551}.
\newblock


\bibitem[\protect\citeauthoryear{Zhang, Zou, and Ma}{Zhang
  et~al\mbox{.}}{[n.d.]}]%
        {DBLP:conf/iclr/ZhangZ020}
\bibfield{author}{\bibinfo{person}{Ruochi Zhang}, \bibinfo{person}{Yuesong
  Zou}, {and} \bibinfo{person}{Jian Ma}.} \bibinfo{year}{[n.d.]}\natexlab{}.
\newblock \showarticletitle{Hyper-SAGNN: a self-attention based graph neural
  network for hypergraphs}. \bibinfo{publisher}{ICLR 2020, Addis Ababa,
  Ethiopia, April 26-30, 2020}.
\newblock


\bibitem[\protect\citeauthoryear{Zhang, Lin, Gao, and BNRist}{Zhang
  et~al\mbox{.}}{2018}]%
        {zhang2018dynamic}
\bibfield{author}{\bibinfo{person}{Zizhao Zhang}, \bibinfo{person}{Haojie Lin},
  \bibinfo{person}{Yue Gao}, {and} \bibinfo{person}{KLISS BNRist}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Dynamic Hypergraph Structure Learning.}. In
  \bibinfo{booktitle}{\emph{IJCAI}}. \bibinfo{pages}{3162--3169}.
\newblock


\bibitem[\protect\citeauthoryear{Zhao, Ding, Han, and Gao}{Zhao
  et~al\mbox{.}}{2018}]%
        {zhao2018personality}
\bibfield{author}{\bibinfo{person}{Sicheng Zhao}, \bibinfo{person}{Guiguang
  Ding}, \bibinfo{person}{Jungong Han}, {and} \bibinfo{person}{Yue Gao}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Personality-Aware Personalized Emotion Recognition
  from Physiological Signals.}. In \bibinfo{booktitle}{\emph{IJCAI}}.
  \bibinfo{pages}{1660--1667}.
\newblock


\bibitem[\protect\citeauthoryear{Zheng, Luo, Sun, Ding, and Zhang}{Zheng
  et~al\mbox{.}}{2018}]%
        {zheng2018novel}
\bibfield{author}{\bibinfo{person}{Xiaoyao Zheng}, \bibinfo{person}{Yonglong
  Luo}, \bibinfo{person}{Liping Sun}, \bibinfo{person}{Xintao Ding}, {and}
  \bibinfo{person}{Ji Zhang}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{A novel social network hybrid recommender system
  based on hypergraph topologic structure}.
\newblock \bibinfo{journal}{\emph{World Wide Web}} \bibinfo{volume}{21},
  \bibinfo{number}{4} (\bibinfo{year}{2018}), \bibinfo{pages}{985--1013}.
\newblock


\bibitem[\protect\citeauthoryear{Zhou, Huang, and Sch{\"o}lkopf}{Zhou
  et~al\mbox{.}}{2007}]%
        {zhou2007learning}
\bibfield{author}{\bibinfo{person}{Dengyong Zhou}, \bibinfo{person}{Jiayuan
  Huang}, {and} \bibinfo{person}{Bernhard Sch{\"o}lkopf}.}
  \bibinfo{year}{2007}\natexlab{}.
\newblock \showarticletitle{Learning with hypergraphs: Clustering,
  classification, and embedding}. In \bibinfo{booktitle}{\emph{NeurIPS}}.
  \bibinfo{pages}{1601--1608}.
\newblock


\end{thebibliography}

